Constructive interference at the edge of quantum ergodic dynamics

Quantum observables in the form of few-point correlators are the key to characterizing the dynamics of quantum many-body systems. In dynamics with fast entanglement generation, quantum observables generally become insensitive to the details of the underlying dynamics at long times due to the effects of scrambling. In experimental systems, repeated time-reversal protocols have been successfully implemented to restore sensitivities of quantum observables. Using a 103-qubit superconducting quantum processor, we characterize ergodic dynamics using the second-order out-of-time-order correlators, OTOC$^{(2)}$. In contrast to dynamics without time reversal, OTOC$^{(2)}$ are observed to remain sensitive to the underlying dynamics at long time scales. Furthermore, by inserting Pauli operators during quantum evolution and randomizing the phases of Pauli strings in the Heisenberg picture, we observe substantial changes in OTOC$^{(2)}$ values. This indicates that OTOC$^{(2)}$ is dominated by constructive interference between Pauli strings that form large loops in configuration space. The observed interference mechanism endows OTOC$^{(2)}$ with a high degree of classical simulation complexity, which culminates in a set of large-scale OTOC$^{(2)}$ measurements exceeding the simulation capacity of known classical algorithms. Further supported by an example of Hamiltonian learning through OTOC$^{(2)}$, our results indicate a viable path to practical quantum advantage.

==> permutation_mc.tex <==
{\color{green}Tom: this section has been pulled from the permutation picture analysis. If it stays here, it will need some re-writing as it now comes before some of the permutation picture definitions.}

\sm{This section doesn't follow the same notation used in the previous paragraphs.}

\bw{Rewrite in progress.}

In this subsection, we will motivate possible extensions of the Monte Carlo schemes for OTOC$^{(1)}$ to allow application in approximating OTOC$^{(2)}$ values for individual circuits. 
This extension will be explicitly shown to have a severe sign problem, ruling out another set of classical methods.

To derive this method, it is helpful to reframe the OTOC$^{(1)}$ Monte Carlo schemes from the point of view of the folder operator dynamics, that is the dynamics of two simultaneous copies of the butterfly operator $B(t)^{\otimes 2}.$ If computed exactly, the OTOC can be viewed as a normal correlation function for this two-copy operator:
\begin{equation}
   \OT{(1)} = \Tr\left( B^{\otimes 2}(t) M^{\otimes 2} (\rho \otimes I) \right).
\end{equation}
In the folded picture, the {\it vanilla Monte Carlo} scheme can be viewed as a modification to the evolution of $B^{\otimes 2}(t)$ that projects out off-diagonal pairs of Pauli operators at each site and samples from the diagonal pairs of Pauli operators. In the limit of infinite samples, the Monte Carlo scheme produces an answer equivalent to only projecting out off-diagonal pairs of Pauli operators with no sampling. As described in the main text, this projection is equivalent to replacing the dynamics with the average dynamics of an ensemble of related circuits, where each circuit in the ensemble is identical to the original circuit but with randomly chosen Pauli operator insertions at the locations of the Monte Carlo projections.

For OTOC$^{(2)}$, the natural generalizations of the Monte Carlo scheme is to modify the dynamics of $B^{\otimes 4}(t)$ with projections which implement average ensemble dynamics. If the ensemble is created by inserting random Pauli strings, the four copy operator is projected onto the space of $64$ 4-copy Pauli strings \bw{maybe merge with immediately previous section, as our explanation motivates both the 64-operator Pauli space MC and the permutation space MC.}
If instead the ensemble average is expanded to be to include not just Pauli insertions but arbitrary single qubit gate insertions, taken from a Haar random ensemble, the projection is onto the span of the $4!=24$ operators that permute the $4$ copies of each site. \bw{take citations from average dynamics section}

% In this section, we revisit the permutation dynamics computations for average OTOC$^{(2)}$ with Haar random ensembles of gates, as described in App.~\ref{sec:meanotoc2}. Some attempts to devise sampling strategies for computation of circuit-specific OTOC$^{(2)}$ values may start with 
% a computation of the mean and add in circuit-specific corrections. We show in this section that the sign problem is severe for computing the mean OTOC$^{(2)}$ via sampling the dynamical update rule Eq.~(\ref{eq:scaleddynamics}) for circuits with Haar random two-qubit gates. This provides evidence that the sign problem is a significant roadblock for devising sampling strategies for OTOC$^{(2)}$. On the other hand, the mean OTOC is dominated by a Markovian process; turning this insight into a strategy for sampling individual circuit values is considered in App.~\ref{sec:classical}.

Thus we will try to use Monte Carlo sampling in the basis of the permutation operators to sample the average dynamics of our circuit with Haar random single qubit gate insertions. As our experimental ensembles fix the two-qubit gate choices and only differ in their single qubit gates, the vanilla version of this method, which projects everywhere, will produce identical answers for each circuit in the ensemble and thus not capture any of the fluctuations between circuits. However, as in the case of the $\OT{(1)}$ Monte Carlo methods, it can be improved to capture more fluctuations by doing the projections in fewer spacetime locations.

\bw{Explain the rescaled permutation basis to get rid necessary to get rid of the exponential rescalings from the final state in the 4-copy picture.} 

The average dynamics in the rescaled permutation basis is generated by a transfer operator $\hat{T}^{\sigma_1 \sigma_2}_{\tau_1 \tau_2}$ which can be derived as follows:
\bw{Explain how to derive the transfer operator}
For OTOC$^{(1)}$, this object would be a Markovian update rule; whereas for OTOC$^{(2)}$ it is a dynamics that conserves total weight but with positive and negative update rules, and thus non-Markovian. The question answered in the remainder of the section is whether the signs in this update rule generate a 'severe' sign problem that cannot be overcome by brute force computation. \bw{cite quantum monte carlo methods that sample with positive and negative weights}

Let us consider directly expanding the dynamics
as a sum over permutation basis trajectories
$$
\begin{gathered}
\OT{(2)} = \sum_{\btau} T(\btau) O(\btau),
\\ T(\btau) \equiv \prod_{t=0}^{t_f - 1} \prod_{\langle i, j\rangle \in G(t)} \hat{T}^{\sigma_i^{t+1} \sigma_j^{t+1}}_{\sigma_i^{t}, \sigma_j^{t}},
\end{gathered}
$$
where the trajectory label $\btau = \{ \sigma_1^0, \sigma_1^0, \ldots  \sigma_N^{t_f}\}$ labels each assignment of permutations to all sites and times, $T(\btau)$ labels the weight assigned to this trajectory, and $O(\btau)$ quantifies the effect of the initial and final boundary conditions.
Because of the rescaling of the permutations, we have by construction the conservation of total weight
\begin{equation}
\sum_{\btau} T(\btau) = 1.
\label{eq:pmcweightconservation}
\end{equation}
Additionally, the values $O(\btau)$ are $\mathcal{O}(1)$ constants. It is useful to rewrite the observable as 
$$
\OT{(2)} = \frac{\sum_{\btau} T(\btau) O(\btau)}{\sum_{\btau} T(\btau)}.
$$
The sampling schemes under consideration sample trajectories according to a probability distribution $p(\btau)$ and reweight the trajectories
by $\omega(\btau) = T(\btau)/p(\btau)$, so that 
$$
\OT{(2)} = \frac{\sum_{\btau} p(\btau) \omega(\btau) O(\btau)}{\sum_{\btau} p(\btau) \omega(\btau)} \approx \frac{\sum_{\text{sampled }\btau} \omega(\btau) \mathcal{O}(\btau)}{\sum_{\text{sampled }\btau} \omega(\btau)}.
$$

The severity of the sign problem can be diagnosed by computing the sample variance of the denominator
$$
\text{Var}(\omega) = \sum_{\btau} p(\btau) \omega(\btau)^2 - \left(\sum_{\btau} p(\btau) \omega(\btau)\right)^2 = \langle \omega(\btau)^2 \rangle_{p} - 1,
$$
where $\langle \rangle_{p}$ indicates the average is taken with respect to the distribution $p$. As $\langle \omega \rangle_p = 1$ by construction, a number of samples $N_{s} \sim \text{Var}(\omega)$ is necessary to get an accurate estimate of the denominator. As an example, in the case where 
$$p(\btau) = \frac{|T(\btau)|}{\sum_{\btau} |T(\btau)|},$$
one can show with Eq.~(\ref{eq:pmcweightconservation}) that
$$
\langle\omega^2\rangle_p = \frac{1}{\langle \text{sgn }T(\tau) \rangle_p^2};
$$
so an exponentially large $\langle\omega^2\rangle_p$ exactly corresponds to an exponentially small average sign, which is commonly used as an indicator of the sign problem --- see, for example Ref.~\cite{Troyer2005-kv}.

We use the following incremental sampling algorithm to sample trajectories $\btau$ and corresponding weights $\omega(\btau)$:
\begin{itemize}
    \item Start with an initial configuration $(\sigma^{0}_1, \sigma^{0}_2, \sigma^{0}_3, \ldots )$ and weight $\omega = 1$
    \item Stochastically apply each gate one at a time, replacing $\sigma_i, \sigma_j$  by $\sigma_i', \sigma_j'$ with probability
$$
p^{\sigma_i' \sigma_j'}_{\sigma_i \sigma_j} = \frac{|\hat{T}^{\sigma_i' \sigma_j'}_{\sigma_i \sigma_j}|}{ \sum_{\sigma_i' \sigma_j'} |\hat{T}^{\sigma_i' \sigma_j'}_{\sigma_i \sigma_j}| }.
$$
\item  Update the weight variable $$\omega \leftarrow \omega \frac{\hat{T}}{p} = \omega\, \text{sgn} \left(\hat{T}^{\sigma_i' \sigma_j'}_{\sigma_i \sigma_j} \right)  \sum_{\sigma_i' \sigma_j'} |\hat{T}^{\sigma_i' \sigma_j'}_{\sigma_i \sigma_j}|.$$
\end{itemize}


At each step, the weight of the trajectory changes signs and is multiplied by a factor $Z(\sigma_i, \sigma_j) = |\sum_{\sigma_i' \sigma_j'} \hat{T}^{\sigma_i' \sigma_j'}_{\sigma_i \sigma_j}| \geqslant 1$, where $\sigma_i$ and $\sigma_j$ are two permutations at the current location of a gate. One may expect then that the trajectory weights grow exponentially in magnitude with the number of applied gates. In practice, the growth is much slower than this implies for the following reason: $Z(\sigma_i, \sigma_j) = 1$ whenever $\sigma_i = \sigma_j$, and typical trajectories under this sampling scheme produce a large growing domain of a single permutation that expands at the butterfly velocity, as illustrated in Fig.~\ref{fig:permutation_monte_carlo}~(a). Thus, only gates in the region of the operator front contribute to the growth of weights $\langle \omega(\tau)^2 \rangle_p$ and the severity of the sign problem.

Numerical results for the growth of the sign problem in circuit geometries comparable to the experiment are shown in Fig.~\ref{fig:permutation_monte_carlo}~(b-c). Due to the repeated random multiplications that govern the growth of the weights, the weights follow a log-normal like distribution whose mean grows with depth of the circuit. The magnitude of this growth is rapid for $q=2$, producing astronomically sized weights. The mean value of $\langle \omega^2 \rangle_p$ is shown for a sample of $10^5$ trajectory simulations --- however, due to the extremely broad tails in the distribution of $\omega$, the sample mean is dominated by the largest samples. Nonetheless, the conclusion is clear. With the number of samples needed for convergence $N \sim \langle \omega^2 \rangle \sim 10^{80}$ for realistic circuit geometries, permutation basis sampling is intractable for computing the mean OTOC$^{(2)}$ and thus not a practical starting point for approximating circuit-specific OTOC$^{(2)}$ values.


\begin{figure*}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/nice_looking_traj.pdf}
    \includegraphics[width=0.32\textwidth]{figures/signproblem_severity_2Dhaar_vs_q.pdf}
    \includegraphics[width=0.32\textwidth]{figures/weight_hist_2D_q2_vs_time.pdf}
    \caption{\sm{a, b, c should appear close to the plots} \textbf{Selected results from running permutation basis sampling for computing mean OTOC$\boldsymbol{^{(2)}}$ in a 2D brickwork circuit with Haar random two-qubit gates.}
    The butterfly operator $O$ is chosen as a Pauli $Z$ on a corner qubit. {\bf a}, A typical snapshot produced by the algorithm, on a $40 \times 40$ lattice with a circuit depth of $d=20$. Different colors correspond to different permutations -- a typical trajectory has a single large domain behind the operator front. {\bf b}, Second moment of the weights for a sample of $10^5$ trajectories on a $10 \times 10$ lattice with depths up to $24$, comparable to the experimental geometry. The weights grow rapidly with depth for $q=2$, signaling a severe sign problem. As the local Hilbert space dimension $q$ is increased, the sign problem is increasingly less severe, which can be attributed to a narrowing of the front volume. {\bf c}, A large fraction of the distribution approaches a log-normal distribution with a mean that increases with depth. As the moments of a log-normal distribution are dominated by the far tails, the second moment estimates in ({\bf b}) are noisy.
    }
    \label{fig:permutation_monte_carlo}
\end{figure*}

% In addition Fig.~\ref{fig:permutation_monte_carlo}~(b) shows results with values of $q>2$, where $q$ is the local Hilbert space dimension. As $q$ is increased, the growth rate in the weights $\omega^2$ drops rapidly, approximately proportional to $1/q^2$. As $q$ is increased, the operator front becomes much narrower --- see Eq.~\ref{eq:haarvbD}. The narrowing of the front slows the growth of the weights.
